Auditable Restoration of Distributed Programs

We focus on a protocol for auditable restoration of distributed systems. The need for such protocol arises due to conflicting requirements (e.g., access to the system should be restricted but emergency access should be provided). One can design such systems with a tamper detection approach (based on the intuition of "break the glass door"). However, in a distributed system, such tampering, which are denoted as auditable events, is visible only for a single node. This is unacceptable since the actions they take in these situations can be different than those in the normal mode. Moreover, eventually, the auditable event needs to be cleared so that system resumes the normal operation. With this motivation, in this paper, we present a protocol for auditable restoration, where any process can potentially identify an auditable event. Whenever a new auditable event occurs, the system must reach an "auditable state" where every process is aware of the auditable event. Only after the system reaches an auditable state, it can begin the operation of restoration. Although any process can observe an auditable event, we require that only "authorized" processes can begin the task of restoration. Moreover, these processes can begin the restoration only when the system is in an auditable state. Our protocol is self-stabilizing and has bounded state space. It can effectively handle the case where faults or auditable events occur during the restoration protocol. Moreover, it can be used to provide auditable restoration to other distributed protocol.

==> corruption.tex <==
%\vspace{-2mm}
\section{The corruption of otsn and ctsn}
\label{sec:cor}
%\vspace{-2mm}

In this section we discuss how to prevent the corruption of the $otsc$ and $tcsn$ values. First, we discuss the case where $otsn$ is subject to transient faults and how to prevent such faults in Section \ref{sec:otsncorr} and then explain $ctsn$ corruption in Section \ref{sec:ctsncorr}.

\subsection{otsn Corruption}
\label{sec:otsncorr}

The variable $otsn$ may get corrupted by transient faults and its value can be (1) increased or (2) decreased to an incorrect value. Next, we explain what would happen in each case and how to prevent such corruptions.

\noindent {\bf Incorrect increase of otsn. } If a transient fault increases $otsn$, a false alarm would happen. In other words, the system would go into $S2$ and, hence, the reset will be called unnecessarily. Although this issue does not endanger the system, it is slowing down the performance of the system. To prevent this corruption, we can add sufficient redundancies into the program similar to that in \cite{castroL02}. Thus, the value of $otsn$ cannot be changed.

\noindent {\bf Incorrect decrease of otsn. } Decrementing $otsn$ by a transient fault, the effects would be more significant than that of incorrect incrementing of $otsn$. For instance, assume transient faults decrements $otsn$ by 1. As a result, if \aus are detected, incrementing $otsn$ will remain hidden and the other processes do not get notified of the \aus and the \aus will be lost. To prevent this corruption, we can use the idea of {\em append-only log} (e.g., \cite{venti02}). Using this idea, we need to separate the storage $otsn$ values from the index used to locate the values. In particular, $otsn$ values are stored in an append-only log on a RAID array of disk drives. The simplicity of the append-only log structure eliminates many possible software errors that might cause data corruption and facilitates a variety of additional integrity strategies. A separate index structure allows the $otsn$ values to be efficiently located in the log. However, the index can be regenerated from the data log if required and thus does not have the same reliability constraints as the log itself.


\subsection{ctsn Corruption}
\label{sec:ctsncorr}

Similar to $otsn$, the variable $ctsn$ may also be subject to transient faults. This variable may gets either increased or decreased by the faults. The effects of increasing (respectively decreasing) $ctsn$ is similar to the effects of decreasing (increasing) $otsn$. Moreover, we can utilize the technique explained above for preventing incorrect increments (decrements) of $otsn$ to prevent incorrect decrements (increments) of $ctsn$.



==> definition.tex <==
\section{\Ar}
\label{sec:def}

This section defines the notion of \ar.


==> discussion.tex <==
\section{Discussion}
\label{sec:disc}	



==> problem.tex <==
\section{Problem Statement}
\label{sec:problem}

This section explains why we need a new type of architecture for and define the problem formally.


==> reset.tex <==
\section{\DS Stabilizing Distributed Reset}
\label{sec:reset}
%\vspace{-2mm}

In this section we explain our proposed \ds stabilizing distributed reset program.

The \ds reset program is required to provide the following functionalities: (1) in any arbitrary state where no process has been tampered with, the system reaches a state from where subsequent reset operation completes correctly, (2) in any arbitrary state where some process is tampered with, eventually all processes are aware of this tampering, (3) some process in the system can detect that all processes have been aware of the tampering, and (4) the process that knows all processes are aware of the tampering starts a new reset operation.

Each process $j$ maintains the following variables:

\begin{itemize}
\item $P.j$, which shows the parent of process $j$;
\item $st.j$, which indicates the state of process $j$. This variable can have three different values: {\em reset}, {\em normal}, $\bot$, and $\top$. If there is no tampering, $st.j$ illustrates whether $j$ is in the middle of a reset operation ({\em reset}), or it has completed its last reset operation ({\em normal}). The program utilizes $\bot$ and $\top$ to notify all processes of the tampering;
\item $sn.j$, where denotes a sequence number to distinguish between different reset waves;
\item $otsn.j$???
\item $ctsn.j$???
\item $result$, which helps to detect if all processes participated in the current reset/tampering wave.
\end{itemize}


The program has 12 actions. The first four actions are the standard actions from \cite{tcAroraG94}. Specifically, in action $DR1$, the root process initiates a distributed reset, marks its state as {\em reset}, resets its local state, and propagates a reset wave to its children. When a process $j$ receives a reset wave from its parent, in action $DR2$, $j$ marks its state as {\em reset}, resets its local state, and propagates the reset wave to its children. When a leaf process $j$ receives a reset wave, $j$ resets its state, marks its state as {\em normal}, and responds to its parent. In action $DR3$, when the root receives the response from its children, the {\em reset} wave is complete.
Action $DR3$ also detects if all processes participated in the current reset wave. This detection is made possible by letting each process maintain the variable {\em result} that is false only if its neighbors have propagated that wave. In particular, if process $j$ has completed a reset wave with result true, then the parent of $j$ completes that reset wave with the result true. It follows that when the root completes the reset wave with the result false, all processes have participated in the reset wave.
To represent action $DR4$, first, we define $Gd.j$ as follows:

\begin{tabbing}
$Gd.j =$\\
\hspace*{4mm} $(((st.(P.j) = reset \wedge st.j = reset) $\\ 
\hspace*{4cm} $ \vee \ (st.(P.j) = \bot \wedge st.j = \bot))$\\
\hspace*{10mm} $\Rightarrow$\\
\hspace*{4mm} $sn.j = sn.(P.j) \wedge otsn.j = otsn.(P.j) $\\ 
\hspace*{4cm} $ \wedge \ ctsn.j = ctsn.(P.j)) \ \ \ \ \ \wedge $\\

\hspace*{4mm} $((st.(P.j) \neq reset \wedge st.(P.j) \neq \bot)$\\
\hspace*{10mm} $\Rightarrow$\\
\hspace*{4mm} $(st.j \neq reset \wedge st.j \neq \bot \wedge sn.j = sn.(P.j) $\\
\hspace*{4cm} $\wedge \  otsn.j=otsn.(P.j))) \ \ \ \ \wedge$\\

\hspace*{4mm} $(((st.(P.j) = \top \wedge st.j = \top)$\\ 
\hspace*{10mm} $\Rightarrow$\\
\hspace*{4mm} $(otsn.j = otsn.(P.j) \wedge (sn.j = sn.(P.j)))))$
\end{tabbing}

\iffalse
\begin{tabbing}
$Gd.j = ((st.(P.j) = reset \wedge st.j = reset) $\\
\=\= \hspace*{3.4cm} $\Rightarrow sn.j = sn.(P.j)) \ \ \wedge $\\
\hspace*{12mm}$ ((st.(P.j) \neq reset)$\\
\=\= \hspace*{3.4cm} $\Rightarrow (st.j \neq reset \wedge sn.j = sn.(P.j)))$
\end{tabbing}
\fi

Action $DR4$ guarantees the self-stabilization of the protocol by ensuring that no matter what the initials state is, the program can recover to legitimate states from where future reset operations work correctly. (Explain the faults and fault tolerance here!)

Actions $DR5-DR12$ are for notifying all the processes in the system about tampering of some process in the system and resetting the system.
As mentioned above, each process has some mechanism that detects the tampering. If a tampering is detected, the process $j$ increases it $otsn.j$ and propagates it towards the root. In action $DR5$, when the parent of process $j$ observes the change in the $otsn$ of one of its children, it also changes its $otsn$ and forwards it towards the root process. Note that, if there is a reset wave propagating in the system while a tampering a detected, that reset wave will be failed. When the root process is notified of the tampering, in action $DR6$, it changes its state to $\bot$ and propagates $\bot$ towards its children. Action $DR7$ propagates $\bot$ towards the leaves. When a leaf receives $\bot$, it changes its state to $\top$ and propagates it towards the root. Consider that, similar to action $DR3$, action $DR8$ checks whether all processes participated in the current $\bot$ wave. If a process detects that one of its neighbors' result variable is true, it propagates it towards the root and the root consequently starts a new $\bot$ wave. When the state of the root process becomes $\top$ and the result is false, the root knows that the state of all processes is $\top$. In other words, the root knows that all processes are aware of the tampering.
However, if the root fails when its state is $\bot$ and some process with state $\top$ becomes the new root, this assumption will be violated. Action $DR10$ guarantees that, even if the root fails, the state of all processes will eventually become $\top$ and the root process will be aware of that.
Finally, actions $DR11$ and $DR12$ check if all the $otsn$ and $ctsn$ variables in the system are in consistent with each other.



%\vspace*{-1mm}
\begin{tabbing}
\noindent\rule{0.48\textwidth}{1pt}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% REVISED ORIGINALS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

${\bf DR1}:: P.j = j \wedge st.j = normal \wedge $\\
\=\= \hspace*{0.75cm} \{{\em j needs to initiate a new reset wave}\}\\
\=\= \hspace*{0.75cm} \=  $\longrightarrow st.j,sn.j := reset, sn.j+1;$ {\it \{reset local state of $j$\}}\\\\


${\bf DR2}:: st.(P.j) = reset \wedge sn.j \neq sn.(P.j) \wedge otsn.j=ctsn.j$\\
\>\>\> $\longrightarrow st.j, sn.j, ctsn.j := reset, sn.(P.j),$\\
\>\>\> \hspace*{6mm} $max(ctsn.j, ctsn.(P.j));$  \hspace*{1mm} {\it \{reset local state of $j$\}}\\\\


${\bf DR3}::st.j = reset \wedge (\forall k: P.k = j: sn.j = sn.k \wedge$\\
\>\>\> $ st.k = normal)) \wedge (\forall k: k \in Nbr.j: sn.j=sn.k) $\\

\>\>\>  $\longrightarrow st.j := normal,$\\
\>\>\> \hspace*{6mm} if ($\exists k: k \in Nbr.j \cup \{j\}: result.k \neq 0$) then\\
\>\>\> \hspace*{11mm} if ($P.j = j$) then \\
\>\>\> \hspace*{16mm} $st.j, sn.j := reset, sn.j+1$\\
\>\>\> \hspace*{11mm} else $result.(P.j) := 1$\\
\>\>\> \hspace*{6mm} else if ($P.j = j$) then \{reset is complete\}\\
\>\>\> \hspace*{6mm} $result.j := 0$\\\\

${\bf DR4}:: \neg Gd.j$\\
\>\>\> $\longrightarrow st.j,sn.j,otsn.j,ctsn.j :=$\\
\>\>\> \hspace*{11mm} $st.(P.j),sn.(P.j),otsn.(P.j),ctsn.(P.j)$\\\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RESET %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

${\bf DR5}:: (st.j = normal \vee st.j = reset) \ \wedge$\\
\=\= \hspace*{0.75cm} \= $(\exists k: P.k=j \wedge otsn.k > ctsn.k)$\\
\=\= \hspace*{0.75cm} \= $\longrightarrow  otsn.j := otsn.k$\\\\


${\bf DR6}:: P.j = j \wedge otsn.j \neq ctsn.j \ \wedge$ \\
\>\>\> $(st.j= normal \vee st.j=reset)$\\
\>\>\> $\longrightarrow st.j := \bot$\\\\


${\bf DR7}:: st.j \neq \bot \wedge st.j \neq \top \wedge st.(P.j) = \bot$\\
\>\>\> $\longrightarrow st.j, otsn.j := \bot, max(otsn.j, otsn.(P.j))$\\\\


${\bf DR8}:: st.j = \bot \wedge (\forall k: P.k = j: otsn.k=otsn.j \ \wedge$\\
\>\>\> $st.k = \top) \wedge (\forall k: k \in Nbr.j: sn.j=sn.k) $\\

\>\>\> $\longrightarrow st.j := \top,$\\
\>\>\> \hspace*{6mm} if ($\exists k: k \in Nbr.j \cup \{j\}: result.k \neq 0$) then\\
\>\>\> \hspace*{11mm} if ($P.j = j$) then \\
\>\>\> \hspace*{16mm} $st.j, sn.j := \bot, sn.j+1$\\
\>\>\> \hspace*{11mm} else $result.(P.j) := 1$\\
\>\>\> \hspace*{6mm} else if ($P.j = j$) then $ctsn.j = otsn.j$\\ %\{$\forall j: st.j = \top$\}
\>\>\> \hspace*{6mm} $result.j := 0$\\\\


${\bf DR9}:: P.j = j \wedge \ st.j = \top \wedge ctsn.j=otsn.j$\\
\>\>\> $\longrightarrow st.j, sn.j := reset, sn.j+1$;\\
\>\>\> \hspace*{6mm} {\it \{reset local state of $j$\}}\\\\


${\bf DR10}:: P.j = j \wedge otsn.j > ctsn.j \wedge st.j = \top$\\
\>\>\> $\longrightarrow sn.j, st.j := sn.j+1, \bot$\\\\


${\bf DR11}::otsn.j < otsn.k \longrightarrow otsn.j = otsn.k$\\\\

${\bf DR12}::ctsn.j < ctsn.k \longrightarrow ctsn.j = ctsn.k$\\

\noindent\rule{0.48\textwidth}{1pt}\\
\end{tabbing}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PROOF OF CORRECTNESS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Correctness for \Ds Stabilizing Distributed Reset Program}
\label{sec:proofdr}

$S1: GD \wedge (\forall k: st.k=normal)$

$S2: \forall k: st.k = \top $

$T: ???$


\begin{theorem}[Closure of S1]
The invariant $S1$ is closed under the execution of the system.
\end{theorem}

\begin{proof}
The proof is similar to that in \cite{tcAroraG94}.
\end{proof}

\begin{theorem}[Convergence to S1] \label{lbl:s1}
Upon starting at an arbitrary state in the absence of tampering, the system is guaranteed to reach a state in $S1$.
\end{theorem}

\begin{proof}
The proof is similar to that in \cite{tcAroraG94}.
\end{proof}

\begin{theorem}[Convergence to $S2$]
Upon starting at an arbitrary state in the presence of tampering where $(\exists j: (x=otsn.j) > max(ctsn.j)$), the system is guaranteed to reach a state in $S2$, where ($\forall k: otsn.k \geq x $).
\end{theorem}

\begin{proof}
To prove this theorem, we need to show that, even in the presence of faults, the system converges to $S2$. To this end, we consider the following cases:

\begin{enumerate}
\item The system is guaranteed to converge to $S2$ in the absence of faults;
\item The system converges to $S2$ even if a node fails, and
\item If the node failed is the root process, the system is still guaranteed to converge to $S2$.
\end{enumerate}

To show that case 1 is always true, we need to show that the root process will be notified if there is a tampering in the system and consequently all processes will be notified of this tampering. Detecting tampering, a process increments its $otsn$ and broadcasts it towards the root process by utilizing action $DR5$. Assume that the $otsn$ wave is not at the root yet and the root process has started a new reset wave. We need to show that this reset wave will get lost and the root process will eventually find out about the tampering. Broadcasting the reset wave, a process, say $j$, resets its local state only if $otsn.j=ctsn.j$ (action $DR2$). Thus, a reset wave gets stuck at process $j$ if process $j$ is already notified of tampering, i.e., $otsn.j>ctsn.j$. Additionally, $P.j$ increments its $otsn$ when it observes $otsn.j$ by executing action $DR5$. Finally, the root process executes action $DR6$, increments its $otsn$ and changes its state to $\bot$. Broadcasting the $\bot$ towards the leaves, if a new tampering is detected, it gets lost since the root is aware of the tampering and is notifying all the other processes in the system of the tampering. When a leaf process gets aware of the tampering, it changes its state to $\top$ and broadcasts it towards the root process. Finally, the root process changes its state to $\top$ when all its children have changed their states to $\top$. Note that, the $\top$ wave cannot get broken and the root will eventually receive it. Therefore, in the absence of faults, it is guaranteed that all the processes will be notified of the tampering and the system converges to $S2$.

In case 2, we assume that, in addition to tampering, the system is also in the presence of faults. A process may fail when its state is normal, reset, $\bot$, or $\top$. If the state of the process failed is normal or reset, a tree construction algorithm (e.g., \cite{}) can be used to repair the tree. Also, action $DR3$ guarantees that the reset wave completes correctly. In this action, the root get notified of the failed process by utilizing the variable $result$. If $result$ is true, the root starts a new reset wave. However, if a process fails when a tampering is detected, it cannot connect to them tree till the system is recovered to a normal or reset state. ***NEED TO REVISE THIS PARA**

Similarly, as stated in case 3, the root process may also fail. It the root fails when its state is normal or reset, the neighbors of the root process will find out and will notify the new root about the failure by setting their $result$ variable to true. Therefore, the new root starts a new reset utilizing action $DR8$. If the root fails when its state is $\bot$, the state of the other processes may be normal, reset, $\bot$, or $\top$. If a process with state normal/reset becomes the root, there is at least one process in the system whose $otsn$ is greater than its $ctsn$. Consequently, using actions $DR5$ and $DR6$ the root process gets notified about the tampering and changes its state to $\bot$. Consider that, if the new root is the process detected the tampering, its $otsn$ is greater than it $ctsn$ and, hence, executing action $DR6$ changes its state to $\bot$. Having a process with state $\bot$ as a new root, all processes will eventually change their state to $\top$. If the state of the new root, say $j$, is $\top$, $j$ assumes that the state of all the other processes in the system is also $\top$. However, this is not true since the state of the root failed was not $\top$ and, hence, there may be some processes whose states is not $\top$ either. Action $DR10$ detects whether the state of all processes is $\top$ utilizing the guard $otsn.j>ctsn.j$. If the root becomes $top$ by executing action $DR8$, its $otsn$ would be equal to its $ctsn$ by executing the statement $ctsn:=otsn$ in $DR8$. Nevertheless, if the old root has failed and a new root has become the root by a tree construction program, the guard $otsn.j>ctsn.j$ in action $DR10$ becomes true and the root changes its state to $\bot$ and broadcasts it towards the leaves. This guarantees that if the state of the root is $\top$, the state of all processes is also $\top$. If the root fails when its state is $\top$, the system is already in $S2$ and the state of all the other processes is also $\top$.

*IS REPAIR ALLOWED IN THE RESET WAVE?*\\
*IF THE ROOT DETECTS THE TAMPERING AND FAILS IMMEDIATELY, THE TAMPERING WILL GET LOST*
\end{proof}


\begin{theorem}
Starting from a state in $S2$, the following expression holds: ($\forall k: otsn.k \geq otsn.j$).
\end{theorem}

\begin{proof}
When a process detects a tampering, it increments its $otsn$. All other processes also get notified of the tampering by executing either action $DR7$ or action $DR11$. When a process wants to change its state to $\top$, it needs to check whether its $otsn$ is equal to all its children's $otsn$. This necessity is checked by $\forall k: P.k = j: otsn.k=otsn.j$ in action $DR8$. Therefore, when the state of the root process becomes $\top$, its $otsn$ is equal to its children's $otsn$, thereby satisfying the theorem.
\end{proof}



\begin{theorem}[Convergence to $S1$ from $S2$]
Upon starting at an arbitrary state in $S2$ where ($P.j = j \wedge sn.j = x$), the system is guaranteed to reach a state in $S1$ where ($\forall k: st.k = normal \wedge sn.k > x$).
\end{theorem}

\begin{proof}

We consider the following cases to prove this theorem:
\begin{itemize}
\item The system is guaranteed to converge to $S1$ in the absence of faults, and
\item The system converges to $S1$ even in the presence of faults.
\end{itemize}

When the system is in $S2$, the state of the root is $top$ and its $otsn$ is equal to its $ctsn$. Thus, the root starts a new reset wave by executing action $DR9$. This wave will eventually reset all the states by executing actions $DR12$ and $DR3$. Also, execution of action $DR3$ sets all states back to normal, thereby satisfying case 1. Moreover, if a process fails, action $DR3$ utilizes the variable $result$ to notify the root to reset the system again. This guarantees the convergence to $S1$.

\end{proof}








\iffalse
{\bf Properties. }

\begin{enumerate}
\item $(\exists j: otsn.j > ctsn.j) \wedge sn.j = x$ (for some $x \in N$)\\
\hspace*{6mm} $\Rightarrow \Diamond(\forall k: st.k = \top \wedge sn.k > x)$

\item $ P.j = j \wedge st.j = \top \wedge sn.j = x$\\
\hspace*{6mm} $\Rightarrow \Diamond(\forall k: st.k = normal \wedge sn.k > x) $

\item $ P.j = j \wedge st.j = \top \wedge sn.j = x$\\
\hspace*{6mm} $\Rightarrow \Diamond(\forall k: otsn.k \geq otsn.j) $

\end{enumerate}
\fi































\iffalse
\vspace*{-1mm}
\begin{tabbing}
$DR1:: j$ is a root $\wedge \ st.j = normal \wedge $ \{ j needs to initiate a new reset wave\}\\
\=\= \hspace*{1.5cm} \=  $\longrightarrow st.j,sn.j := reset, sn.j+1;$ {\it \{reset local state of $j$\}}\\\\


$DR2:: st.(P.j) = reset \wedge sn.j \neq sn.(P.j) \wedge st.j \neq tampered$\\
\>\>\> $\longrightarrow st.j, sn.j := reset, sn.(P.j);$ {\it \{reset local state of $j$\}}\\\\


$DR3::st.j = reset \wedge (\forall k: P.k = j: sn.j = sn.k \wedge st.k = normal))$\\
\>\>\> $\wedge (\forall k: k \in Nbr.j: root.j = root.k \wedge sn.j=sn.k) $\\

\>\>\>  $\longrightarrow st.j, tsn.j := normal, sn.j$\\
\>\>\> \hspace*{6mm} if ($\exists k: k \in Nbr.j \cup \{j\}: new.k > 0$) then\\
\>\>\> \hspace*{11mm} if ($P.j = j$) then \\
\>\>\> \hspace*{16mm} $st.j, sn.j := reset, sn.j+1$\\
\>\>\> \hspace*{11mm} else $new.(P.j) := max(new.(P.j), 1)$\\
\>\>\> \hspace*{6mm} else if ($P.j = j$) then \{reset is complete\}\\
\>\>\> \hspace*{6mm} $new.j := max(0, new.j -1)$\\\\


\noindent\rule{15cm}{1pt}\\


$DR4:: (st.j = normal \vee st.j = reset) \wedge (\exists k: P.k=j \wedge st.k = tampered)$\\
\>\>\> $\longrightarrow st.j := tampered$\\\\


$DR5:: P.j = j \wedge st.j = tampered \longrightarrow st.j, tsn := \bot, tsn+1$\\\\


$DR6:: st.j \neq \bot \wedge st.j \neq \top \wedge st.(P.j) = \bot \wedge tsn.(P.j) \neq tsn.j \longrightarrow st.j, tsn.j := \bot, tsn.(P.j)$\\\\


$DR7:: st.j = \bot \wedge (\forall k: P.k = j: tsn.k=tsn.j \wedge st.k = \top)$\\
\>\>\> $\wedge (\forall k: k \in Nbr.j: root.j = root.k \wedge tsn.j=tsn.k) $\\

\>\>\> $\longrightarrow st.j := \top,$\\
\>\>\> \hspace*{6mm} if ($\exists k: k \in Nbr.j \cup \{j\}: new'.k > 0$) then\\
\>\>\> \hspace*{11mm} if ($P.j = j$) then \\
\>\>\> \hspace*{16mm} $st.j, tsn.j := \bot, tsn.j+1$\\
\>\>\> \hspace*{11mm} else $new'.(P.j) := max(new'.(P.j), 1)$\\
\>\>\> \hspace*{6mm} else if ($P.j = j$) then \{We conclude that $\forall j: st.j = \top$\}\\
\>\>\> \hspace*{6mm} $new.j := max(0, new'.j -1)$\\\\


$DR8:: P.j = j \wedge \ st.j = \top $\\
\>\>\> $\longrightarrow st.j, sn.j := reset, sn.j+1;$ {\it \{reset local state of $j$\}}\\\\


$DR9::\neg Gd.j \longrightarrow sn.j = sn.(P.j)$\\\\

\noindent\rule{15cm}{1pt}\\

\end{tabbing}


\noindent {\bf Properties. }

\begin{enumerate}
\item $(\exists j: st.j = tampered) \wedge sn.j = x$ (for some $x \in N$) $\Rightarrow (\forall k: st.k = \top) \wedge (\exists k: tsn.k > x)$
\item $ P.j = j \wedge st.j = \top \wedge sn.j = x \Rightarrow (\forall k: st.k = normal \wedge sn.k > x) $

\end{enumerate}


\noindent\rule{0.48\textwidth}{1pt}\\

\noindent {\bf Fault and Adversary Actions.}\\
\noindent $DR_{adv}:: (st.j = reset \vee st.j = normal) \longrightarrow st.j := tampered $

\noindent $Fail-stop :: up.j \longrightarrow up.j = false; (\forall k: k \in Nbr.j: new.k:=2) $

\noindent\rule{0.48\textwidth}{1pt}\\

\begin{theorem}
\label{thm:reset}
The distributed reset program $DR$ is \emph{\ds stabilizing} with adversary $DR_{adv}$ for \emph{invariants} $\br{S1_{dr},S2_{dr}}$ in environment $U_{dr}$.
\end{theorem}
\fi



\iffalse

\noindent {\bf Proof of Correctness.}

We need to show that starting at any state the system is guaranteed to eventually

\begin{enumerate}
\item reach S1 if there is no tampering in the system. S1 is a steady state that satisfies ($\forall j: sn.j=tsn.j =n \wedge st.j = normal$) for some integer $n$;
\item reach S2 from $\neg T$ if there is tampering in the system. In S2 all processes are notified of occurrence of the tampering, and
\item reach $T$ (or S1??) from S2.
\end{enumerate}

The proof of (1) consists showing that:
\begin{itemize}
\item Starting at any arbitrary state in $T$, the system is guaranteed to reach a state in S1, where ($\forall j:sn.j=tsn.j=n \wedge st.j=normal$), and
\item S1 is closed under system execution.
\end{itemize}

The proof of (2) consists showing that:
\begin{itemize}
\item Starting at any arbitrary state in $\neg T$, the system is guaranteed to reach a state in S2, where all processes are notified of occurrence of the tampering, and if the root process $k$ has $sn.k = n$ and $tsn.k = m$ for some $n$ and $m$, the system is guaranteed to reach a state in ($\forall j:sn.j=n \wedge st.j=\top \wedge tsn.j=m$) (?????);
\item $\neg T$ is closed under system execution (??????Is it true);
\end{itemize}

The proof of (3) consists showing that:
\begin{itemize}
\item Starting at any arbitrary state in S2, the system is guaranteed to reach a state in $T$ (or S1???), where the state of all processes is $reset$;
\item $T$ is closed under system execution;
\end{itemize}



\vspace*{9mm}
\noindent {\bf What happens if tree changes some node's parents from A to B?}

\fi




